Mining Novel Multivariate Relationships in Time Series Data Using Correlation Networks

In many domains, there is significant interest in capturing novel relationships between time series that represent activities recorded at different nodes of a highly complex system. In this paper, we introduce multipoles, a novel class of linear relationships between more than two time series. A multipole is a set of time series that have strong linear dependence among themselves, with the requirement that each time series makes a significant contribution to the linear dependence. We demonstrate that most interesting multipoles can be identified as cliques of negative correlations in a correlation network. Such cliques are typically rare in a real-world correlation network, which allows us to find almost all multipoles efficiently using a clique-enumeration approach. Using our proposed framework, we demonstrate the utility of multipoles in discovering new physical phenomena in two scientific domains: climate science and neuroscience. In particular, we discovered several multipole relationships that are reproducible in multiple other independent datasets and lead to novel domain insights.

==> Introduction/IntroductionAug2018OLD.tex <==
\IEEEraisesectionheading{\section{Introduction}\label{sec:Intro}}
% \section{Introduction}\label{Sec:Intro}
\IEEEPARstart{I}{n} many domains, understanding the relationships between time series is essential for obtaining actionable insights. For instance, in climate science, pressure dipoles, which are pairs of locations with strong negative correlations in their Sea Level Pressure time series, have been extensively studied, and have been linked with anomalous weather events all over the globe such as forest fires, hurricanes etc.\cite{kawale2013graph,taschetto2014cold,wallace1981teleconnections}. Similarly, in neuroscience, researchers have discovered pairs of brain regions that exhibit positive correlations between their activity time series. These correlated time series represent brain regions exhibiting synergistic activity \cite{atluri2016brain}.

%\begin{figure*}[t]
%\centering
%\begin{subfigure}[t]{0.25\textwidth}
%\includegraphics[width=\textwidth]{Introduction/Figs/variance_0}
%\centering
%\caption{Variance = 0}
%\label{fig:ldda}
%\end{subfigure}
%\centering
%\begin{subfigure}[t]{0.25\textwidth}
%\includegraphics[width=\textwidth]{Introduction/Figs/variance_decimal02}
%\centering
%\caption{Variance = 0.02}
%\label{fig:lddb}
%\end{subfigure}
%\centering
%\begin{subfigure}[t]{0.25\textwidth}
%\includegraphics[width=\textwidth]{Introduction/Figs/variance_decimal_3}
%\centering
%\caption{Variance = 0.3}
%\label{fig:lddc}
%\end{subfigure}
%\caption{(a) Illustrating measurement of linear dependence between two variables $X$ and $Y$ as variance of their least variant unit-length linear combination. Linear dependence between X and Y decreases from (a) to (c), as the variance of least variant linear combination increases}.
%\label{fig:lin_dep_demo}
%\end{figure*}

In this work, we define a novel class of linear relationships, called \textbf{multipoles}, that involve more than two time series, also referred to as variables.  We say that a set of variables is a multipole if i) the variables show strong linear dependence, and ii) each variable makes a significant contribution to the linear dependence, i.e., excluding any of the variables from the set significantly weakens the strength of the linear dependence among the remaining variables. We define linear dependence in terms of the variance of a linear combination of the standardized (zero mean, unit variance) vectors. We measure the strength of the linear dependence of a set of time series by the variance of their \textit{least variant} linear combination, i.e., a (unit-length) linear combination that has the minimum variance. The smaller the variance of this linear combination, the more constant (less variable) the linear combination, and thus higher the linear dependence, and vice-versa. We define the contribution of each variable to the linear dependence as the reduction in the strength of the linear dependence of the smaller set when this variable is removed. We define linear gain as the minimum contribution of included variables to the linear dependence.   

%measure whether each variable makes a significant contribution in terms of the linear gain, which is essentially

%In this work, we define a novel class of linear relationships, called \textbf{multipoles}, that involve more than two time series.  We say that a set of variables is a multipole if i) the variables show strong linear dependence, i.e., there exists a linear combination of them that is relatively invariant across all the observations, and ii) each variable makes a significant contribution to the linear dependence, i.e., elimination of any of the variables from the set significantly weakens the strength of the linear dependence among the remaining variables. We measure the strength of the linear dependence of a set of time series by the variance of their \textit{least variant} linear combination, i.e. a (unit-length) linear combination that has the minimum variance. The smaller the variance of this linear combination, the more constant (less variable) the linear combination, and thus higher the linear dependence, and vice-versa. (See Figure~\ref{fig:lin_dep_demo} for illustration and Section~\ref{Sec:Def} for precise definitions.) 

We next illustrate multipoles with a real-world example. Consider a set $S$ of three time series $T_1$, $T_2$, and $T_3$, shown in Figure~\ref{fig:rawts}, which capture the traffic volume on three different roads in Minnesota as shown in Figure~\ref{fig:good_map}. The three bottommost plots of Figure~\ref{fig:lc} show the least variant linear combination for each possible pair, while the top plot of Figure~\ref{fig:lc} shows the least variant linear combination for all three. Note that the linear combination of all three time series has a variance of only $0.08$.Thus, we say that there exists a strong, although not perfect, linear dependence among the above three time series.

Further, note that each of the three time series forms a crucial component of the relationship, as excluding any one of them will significantly weaken the strength of the linear dependence among the remaining two time series. For example, if $T_3$ is excluded from the set, the variance of the least variant linear combination $Z_{12}$ of $T_1$ and $T_2$ turns out to be $0.33$, which is much higher than the variance $0.08$ of $Z$, thus indicating a significant contribution from $T_3$. Similarly, if we exclude $T_1$ or $T_2$ instead of $T_3$, the variance of least variant combinations become $0.58$ and $0.74$. (See the three bottommost plots of Figure~\ref{fig:lc}.) The linear gain for $\{T_1, T_2, T_3\}$ is $\min\{0.33, 0.58, 0.74\} - 0.08 = 0.25$.

An explanation for the relationships illustrated above can be provided by the notion of conservation of flow. Two of the time series, $T_1$ and $T_2$, were observed on the roads that act as major tributaries to the highway where $T_3$ is being observed. All the southbound traffic coming from the tributaries is likely to merge at the highway, thus leading to a strong linear dependence among the three time series. Omitting any single time series leads to a weaker linear dependence because, unlike the highway, traffic flow in the tributaries significantly changes during weekends (see peaks and drops every Sunday), which weakens the strength of their pairwise linear relationships with highway. However, the simultaneous rise and fall in traffic on both tributaries complements each other, resulting in a stronger linear dependence among the three time series.

%Multipoles can be observed in several real-world domains. We next illustrate multipoles with a real-world example. Consider a set $S$ of three time series $T_1$, $T_2$, and $T_3$, shown in Figure~\ref{fig:rawts}, which capture the traffic volume on three different roads in Minnesota as shown in Figure~\ref{fig:good_map}. To quantify linear dependence, we considered the least variant linear combination of them, which has a variance of only $0.08$, as shown in the top panel in Figure~\ref{fig:lc}. Thus, we say that there exists a strong, although not perfect, linear dependence among the above three time series. 

%An explanation for this relationship can be provided from the notion of conservation of flow. Two of the time series, $T_1$ and $T_2$, were observed on the roads that act as major tributaries to the highway where $T_3$ is being observed. All the southbound traffic coming from the tributaries is likely to merge at the highway, thus leading to a strong linear dependence among the three time series.

%Further, note that each of the three time series forms a crucial component of the relationship, as excluding any one of them will significantly weaken the strength of the linear dependence among the remaining two time series. For example, if $T_3$ is excluded from the set, the variance of the least variant linear combination $Z_{12}$ of $T_1$ and $T_2$ turns out to be $0.33$, which is much higher than the variance $0.08$ of $Z$, thus indicating a significant contribution from $T_3$. Similarly, if we exclude $T_2$ or $T_3$ instead of $T_1$, the least variances become $0.58$ and $0.74$, respectively, as shown in the bottom two panels of Figure~\ref{fig:lc}. This is due to the fact that unlike the highway, traffic flow in the tributaries significantly changes during weekends (see peaks and drops every Sunday), which weakens the strength of their pairwise linear relationships with highway. However, the simultaneous rise and fall in traffic on both tributaries complements each other, resulting in a stronger linear dependence among the three time series. 

Multipoles can also be seen in other domains. For instance, we used the techniques presented in this paper to find several previously unknown multipole relationships between climate variables observed at more than two distant locations. Similarly, in neuroscience, we found novel multipole relationships between different brain regions that are triggered by specific visual and auditory stimuli. Some of these relationships were found to have insightful domain interpretations. (See  Section~\ref{Sec:PhysInt}.)

The relationships and conditional independence of two or more variables have been widely studied in different contexts using a variety of techniques including regression models \cite{tibshirani1996regression,lozano2009spatial,chatterjee2012sparse,carroll2006measurement}, PCA-based approaches\cite{barnston1987classification,ding2005circumglobal}, structure learning methods \cite{friedman2008sparse,meinshausen2006high}, correlation network analysis \cite{tsonis2011community,donges2009backbone,kawale2011discovering,agrawal2017tripoleslong}, etc. However, as discussed in Section \ref{sec:RelWork}, multipole relationships as defined here can be viewed as novel in the sense that none of these previous approaches can be used to find the type of relationship represented by multipoles in the data. 

%To the best of our knowledge, multipole relationships have never been defined nor systematically studied in the previous literature. The relationships and conditional independence of two or more variables have been widely studied in different contexts using a variety of techniques including regression models\cite{tibshirani1996regression,lozano2009spatial,chatterjee2012sparse,carroll2006measurement}, PCA-based approaches\cite{barnston1987classification,ding2005circumglobal}, structure learning methods \cite{friedman2008sparse,meinshausen2006high}, correlation network analysis \cite{tsonis2011community,donges2009backbone,kawale2011discovering,agrawal2017tripoleslong}, etc. However, none of these approaches can be used to find multipoles in the data. (See Section~\ref{sec:RelWork}.) 

A na\"{\i}ve approach to find all multipoles in a time series dataset would be to enumerate all possible combinations of time series and measure the strength of their linear dependence and linear gain. However, this is computationally infeasible due to the combinatorial nature of the search space. In this paper, we present an efficient approach to find multipoles.

%A na\"{\i}ve approach to find all multipoles in a time series dataset would be to enumerate all possible combinations of time series and evaluate their linear dependence and \textit{linear gain}, which is essentially the minimum contribution of included variables to the linear dependence. However, this is computationally infeasible due to the combinatorial nature of the search space. 


This approach formulates the multipole-search problem as a clique-enumeration problem in a correlation network, where each node represents a time series, and the weight of an edge between two nodes represents the strength of the linear correlation between the corresponding time series. Our proposed problem formulation is motivated by the following two key empirical observations: the upper limit on the linear gain of a multipole is dependent on  i) the size of multipole, and ii) the maximum correlation strength among two variables in a multipole. %These observations help us establish that most of the multipoles having high linear gain appear in a correlation network either as \emph{negative cliques}, i.e. sets with all pairwise correlations being negative, or \emph{negative-equivalent cliques}, that can be transformed into negative cliques by flipping the signs of one or more of its member variables (see Definitions~\ref{def:negcl} and \ref{def:pseudo} for further details). 

Leveraging these observations, we propose a novel \textbf{C}lique Based \textbf{M}ultipole S\textbf{e}arch (CoMEt) approach to find most interesting multipoles in a time series dataset. The central idea of the approach is to identify and restrict the search for multipoles to family of subsets, which we refer to as `promising candidates` that are more likely to exhibit multipole relationships with stronger linear gain between their members. Using the above empirical observations,  we show that most promising candidates of multipoles with high linear gain appear in a correlation network either as \emph{negative cliques}, i.e. sets with all pairwise correlations being negative, or \emph{negative-equivalent cliques}, that can be transformed into negative cliques by flipping the signs of one or more of its member variables (see Definitions~\ref{def:negcl} and \ref{def:pseudo} for further details). The number of promising candidates typically turns out to be much smaller in scenarios where multipoles with high linear gain are desired, thereby contributing to the remarkably high computational efficiency of our approach, although with some loss of completeness in the final output. 

Furthermore, we propose CoMEtExtended, a more generalized version of CoMEt approach, where we redefine what constitutes a promising candidate. In particular, CoMEtExtended involves an additional parameter that can be tuned to expand or prune the scope of promising candidates beyond negative cliques and negative-equivalent cliques, which allows one to achieve a better trade-off between computational efficiency and completeness at different thresholds of linear gain (see Section~\ref{Sec:COMETEXT} for further details).
 
%The loss in completeness could be further higher at lower thresholds of linear gain, since many multipoles with weaker linear gain  do not necessarily appear as negative cliques or negative equivalent cliques and consequently get missed. Therefore, to improve completeness at lower thresholds of linear gain, we propose CoMEtExtended, an extended version of our approach, where we generalize the scope of promising candidates to include pseudo-negative cliques, where all the pairwise correlations are allowed to below a threshold instead of being necessarily negative. 


%family of subsets, which we refer to as `promising candidates` that are more likely to exhibit multipole relationships with stronger linear gain between their members. 


%we propose to identify and restrict the search for multipoles to a family of subsets, which we refer to as `promising candidates` that are more likely to exhibit multipole relationships with stronger linear gain between their members. Such a family of subsets are usually much rarer in the data, thereby contributing to the remarkably high computational efficiency of our approach, although with some loss of completeness in the final output of multipoles. 

%Leveraging the above observations, we propose a novel \textbf{C}lique Based \textbf{M}ultipole S\textbf{e}arch (CoMEt) approach to find most interesting multipoles in a time series dataset. The general idea of our approach is to identify and restrict the search space of interesting multipoles to a smaller family of subsets, which we refer to as `promising candidates` that are more likely to exhibit multipole relationships with stronger linear gain between their members. Such a family of subsets are usually much rarer in the data, thereby contributing to the remarkably high computational efficiency of our approach, although with some loss of completeness in the final output of multipoles. 

%Leveraging the above observations, we propose a novel \textbf{C}lique Based \textbf{M}ultipole S\textbf{e}arch (CoMEt) approach to find most interesting multipoles in a time series dataset. In particular, we show that most promising candidates of interesting multipoles can be identified as sets that appear in a correlation network either as \emph{negative cliques}, i.e. sets where all pairwise correlations between its members are negative,  or \emph{negative-equivalent cliques}, i.e. sets that can be transformed into negative cliques by flipping the signs of one or more of its member variables (see Definitions~\ref{def:negcl} and \ref{def:pseudo} for further details).  Although the clique-enumeration problem is NP-complete in general, we observed that cliques of our interest are much smaller in number in a real-world correlation network, which allows us to efficiently find most of the interesting multipoles, although with some loss of completeness in the final output.  

%In this paper, we provide two implementations of CoMEt: CoMEtBasic and Such a family of subsets are usually much rarer in the data, thereby contributing to the remarkably high computational efficiency of our approach, although with some loss of completeness in the final output of multipoles.

%In certain cases, the completeness and computational efficiency of CoMEt might be unsatisfactory. For instance, at lower thresholds of linear gain, the obtained set of promising candidates in CoMEt could potentially miss some of the interesting multipoles. On the other hand, at high thresholds of linear gain, there could potentially be many false positives among promising candidates, which would compromise the computational efficiency. Hence, to overcome these limitations of CoMEt,  we further propose \textit{CoMEtExtended}, a generalized version of CoMEt, which involves an additional parameter that can be tuned to expand or prune the scope of promising candidates beyond negative cliques and negative-equivalent cliques, in order to achieve a better trade-off between computational efficiency and completeness at different thresholds of linear gain.  

%space  we parametrize the notion of \emph{negative clique} to \emph{pseudo negative clique}, which requires all of the pairwise correlations in a set below a threshold $\rho$, where $\rho \in [-1,1]$. The concept of negative equivalent cliques is also modified accordingly (see Definitions~\ref{def:pseudonegcl} and \ref{def:pseudonegeq}). The advantage of CoMEtExtended over CoMEt is that the search space of interesting multipoles can be expanded or pruned by tuning the parameter $\rho$ which allows one to achieve a better trade-off between computational efficiency and completeness.


Our paper makes several key contributions: 1) We formally define multipole, a novel relationship in time series data and devise measures to quantify its interestingness. 2) We formulate a novel and computationally efficient pattern-mining approach to find most interesting multipoles in a time series dataset. 3) Further, we propose an empirical framework to evaluate discovered multipoles that includes an empirical procedure to assess the statistical significance of multipoles. 4) Using our proposed framework, we demonstrate the relevance of multipoles to two scientific domains: climate science and neuroscience.



\begin{figure}[t]%{0.4\textwidth}
\centering
% \includegraphics[scale=0.3]{Introduction/Figs/tripole_good_horizontal.png} 
\includegraphics[scale=0.4]{Introduction/Figs/tripole_horiz.eps} 
\caption{A multipole among daily traffic time series $T_1$,$T_2$, and $T_3$ observed for three roads in Minneapolis}
\label{fig:good_map}
\end{figure}

\begin{figure}[tb]
\centering
\begin{subfigure}[t]{0.24\textwidth}
\includegraphics[width=\textwidth]{Introduction/Figs/TsPlot_KDD_17_tripole_}
\centering
\caption{}
\label{fig:rawts}
\end{subfigure}
\centering
\begin{subfigure}[t]{0.24\textwidth}
\includegraphics[width=\textwidth]{Introduction/Figs/TsPlot_KDD_17_tripole_MCNLC}
\centering
\caption{}
\label{fig:lc}
\end{subfigure}
\caption{(a) Standardized (zero mean and unit variance) daily traffic volume for the three roads shown in Figure~\ref{fig:good_map}. (b) Time series of their linear combinations}
\label{fig:good_tripole}
\end{figure}


==> Methods/EmpiricalBoundsJan2019.tex <==
\subsection{Self-Cancellation}

\begin{definition}\label{Def:SelfCan}
A set is said to be \textbf{self-canceling} if all the weights in its LVNLC are non-negative.
\end{definition}

%In other words, the variables in a self-canceling set tend to cancel each other, due to which their LVNLC has positive weights for all the members. 
Any non self-canceling set $S$ can be converted into a self-canceling set $\widetilde{S}$, by flipping the signs of all the members in $S$ that have negative weights in LVNLC of $S$. For example, consider the set $S\equiv{T_1,T_2,T_3}$ of three traffic time series from transportation example discussed in Section~\ref{sec:Intro}. The LVNLC of $S$ was observed to be $0.6T_1 + 0.65T_2 -0.47T_3$ (see top panel of Figure~\ref{fig:good_tripole}). By flipping the sign of $T_3$, we get a new set $\widetilde{S}\equiv\{T_1,T_2,-T_3\}$, whose LVNLC is given by $0.6T_1 + 0.65T_2 +0.47(-T_3)$. Since all the variables in $\widetilde{S}$ have non-negative weights in its LVNLC, $\widetilde{S}$ is a self-canceling set. It is important to note that flipping the signs of one or more variables does not affect the eigenvalues of their correlation matrix. Therefore, $S$ and $\widetilde{S}$ will have identical linear dependence and linear gain. Based on the above ideas, we can define a canonical form of the set called the \emph{self-canceling form} as the following. 

\begin{definition}\label{Def:SelfCanForm}
A \textbf{self-canceling form} of a set $S$ is a canonical form $\widetilde{S}$ that is obtained by flipping the signs of all the variables that have negative weights in LVNLC of $S$.
\end{definition}

%More formally, an equivalence class of sets can be defined in which any two sets are transformable into one another by flipping the signs of one or more variables in the set. Every equivalence class will then have one self-canceling set which will be the common canonical form of all the sets in that class. 

%Also note that a self-canceling set $\widetilde{S}$ of size $k$ will be the canonical (self-canceling) form of as many as $2^k$ sets (each of them could be derived by considering all possible combinations of sign assignments to the members of $\widetilde{S}$.)

\subsection{Empirical Observations}\label{sec:EmpObs}
We are now in a position to describe our empirical observations that relate linear gain of a set $S$ with largest pairwise correlation in its self-canonical form $\widetilde{S}$. 
Specifically, let \textbf{$\rho_{S}$} denote the highest pairwise correlation observed in $\widetilde{S}$. Figure~\ref{fig:EmpRes} then shows scatter plots between $\Delta\sigma_S$ (X-axis) and $\rho_{S}$ (Y-axis) for more than a million correlation matrices of sizes $k \times k$ for $k = 3,4,5$. Each of these matrices were generated by sampling all $\binom{k}{2}$ pairwise correlations between $[-1,1]$ using a uniform distribution. Among the generated matrices, only the ones that satisfy positive semi-definiteness were considered to be valid correlation matrices. The implementation of the procedure can be accessed at this URL  \footnote{https://github.com/15saurabh16/Multipoles}. From Figure~\ref{fig:EmpRes}, we make two key observations:


%\hyperref[https://github.com/15saurabh16/Multipoles]{\color{red}link}.%\href{https://github.com/15saurabh16/Multipoles}{link}.

%Only f the resultant matrix turns out to be positive semi-definite, it before being considered as a 

%In particular, for $k=3$, all correlation matrices were generated at a numerical resolution of 0.01. However, as size of the correlation matrix grows bigger, it gets computationally infeasible to cover all correlation matrices at higher numerical resolution. Therefore, for $k>3$, we randomly generated a population of around $10^6$ matrices using the following procedure: Each correlation matrix of size $k \times k$ is generated by randomly selecting $\binom{k}{2}$ numbers in the range $[s,e]$ under uniform distribution, where $s\in [-1,1]$ and $e\in [s,1]$, and then arbitrary placing them as the off-diagonal entries in the upper triangular part of the matrix. The lower triangular part is then filled to keep the matrix symmetric.
\begin{figure*}
\centering
\begin{subfigure}[t]{0.30\textwidth}
\centering
% \includegraphics[width = 5cm,height = 4cm]{Methods/Figs/All3-PolesLEVGvsMaxEdge.eps} 
\includegraphics[width = 5cm,height = 4cm]{Methods/Figs/EmpObsSize3} 
\caption{3-Poles}
\label{fig:Emp3}
\end{subfigure}
\begin{subfigure}[t]{0.30\textwidth}
\centering
% \includegraphics[width = 5cm,height = 4cm]{Methods/Figs/All4-PolesLEVGvsMaxEdge.eps}
\includegraphics[width = 5cm,height = 4cm]{Methods/Figs/EmpObsSize4} 
\caption{4-Poles}
\label{fig:Emp4}
\end{subfigure}
\begin{subfigure}[t]{0.30\textwidth}
\centering
% \includegraphics[width = 5cm,height = 4cm]{Methods/Figs/All5-PolesLEVGvsMaxEdge.eps}
\includegraphics[width = 5cm,height = 4cm]{Methods/Figs/EmpObsSize5} 
\caption{5-Poles}
\label{fig:Emp5}
\end{subfigure}
\caption{Empirical relationship between linear gain $\Delta\sigma_S$ of a set $S$ (X-axis)  and largest pairwise correlation in its self-canceling form $\widetilde{S}$ (Y-axis) on more than $10^6$ generated $k \times k$ correlation matrices for $k \in [3,5]$. Vertical red-dash line in each plot indicates largest value of linear gain observed. All promising candidates for CoMEt approach lie below the $\rho_S = 0$ (green solid line). All multipoles with linear gain larger than a given threshold $\delta$  lie to the right of the vertical solid black line.}
\label{fig:EmpRes}
\end{figure*}

\textbf{First key observation:} All the plots in Figure~\ref{fig:EmpRes} show that the sets with largest linear gain (the rightmost end of the distribution) always lie below horizontal green line that corresponds to equation $\rho_S=0$. This implies that the linear gain of a set $S$ tends to be higher when the largest pairwise correlation in $\widetilde{S}$ is strongly negative. More generally, for all sets that form multipoles with linear gain at least $\delta$, there exists an upper bound on the largest pairwise correlation in their self-canceling forms.  
%$\rho$ on $\rho_S$. %Hence, if we are interested in finding multipoles with linear gain at least $\delta$, we can potentially discard all those sets that have at least one pairwise correlation larger than $\rho$ in their self-canceling versions. 

\textbf{Second key observation:}  The maximum possible linear gain of a multipole of size $k$ is $\frac{1}{k-1}$. (In Figure~\ref{fig:EmpRes}, we can see that for $k$ equal to 3,4, and 5, the maximum linear gain is 0.5, 0.33, and 0.25, respectively.) The maximum linear gain corresponds to the set where all the pairwise correlations in its self-canceling version equals $\frac{-1}{k-1}$. This implies that the linear gain is smaller for larger multipoles. Hence, if we are only interested in finding multipoles with linear gain at least $\delta$, we can safely ignore all sets beyond of size $\floor*{\frac{1+\delta}{\delta}}$. Both of the above two observations were found to empirically hold true also for sets of sizes beyond 5. 

Based on the above empirical observations, we next define a promising candidate for a multipole in the following subsection.


%We empirically verified both of the above observations on as many correlation matrices as we could and found out that it always turns out to be true. Specifically, we considered all correlation matrices of $3 x3$ that were generated at a numerical resolution of 0.01. However, as size of the correlation matrix grows bigger, it gets computationally infeasible to cover all correlation matrices at higher numerical resolution. Therefore, we generated a population of around 1,000,000 correlation matrices of size $k \times k$ for $k = 4,5,6$. Each correlation matrix of size $k \times k$ is generated by randomly selecting $k(k-1)/2$ numbers in the range $[s,e]$ under uniform distribution, where $s\in [-1,1]$ and $e\in [s,1]$, and then arbitrary placing them as the off-diagonal entries in the upper triangular part of the matrix. The lower triangular part is then filled to keep the matrix symmetric. The resultant matrix is then checked for positive semi-definiteness before being considered as a valid correlation matrix. 

%Consider a set $S = \{X_1,X_2,...X_k\}$ of $k$ variables. Let $\widetilde{S}$ be the self-canceling set obtained from $S$, and its correlation matrix be $\widetilde{A}$. Then a promising candidate is defined as the following: 

% \begin{definition}
% A set $S$ is said to be a \textbf{promising candidate} if i) $|S| \leq \floor*{\frac{1+\delta}{\delta}}$, where $\delta$ is the user-specified threshold on linear gain, and ii) $\widetilde{A_{ij}}<0,\forall i,j \in [1,|S|],i \neq j$,
% \end{definition}

% In other words, a promising candidate $S$ is one whose maximum size is governed by $\delta$ and all the pairwise correlations among the members of its self-canceling version $\widetilde{S}$ are below 0. 

% We next present our empirical observations that motivate the above definition of promising candidates. 

%We are now in a position to present our empirical bounds on the linear gain of a set. 
%In this section, we present a series of empirical observations that indicate relationship between linear gain of a set of variables and the underlying correlation structure between the variables of the set. As we will discuss further in section~\ref{},all these observations presented in this section could be leveraged to drastically reduce the search-space of interesting multipoles in the data. 

%\subsubsection{Relation with Mean of Pairwise Correlation Strengths}


%Consider a set $S = \{X_1,X_2,...X_k\}$ of $k$ variables. Let $\widetilde{S}$ be the self-canceling set obtained from $S$, and its correlation matrix be $\widetilde{A}$. For such a set $S$, we made following two empirical observations:

% \begin{observation}\label{Obs0}
% The maximum possible linear gain for a set $S$ of $k$ variables is $\leq \frac{1}{k-1}$ that is obtained when all the pairwise correlations in $\widetilde{S}$ are equal to $-\frac{1}{k-1}$. 
% \end{observation}

% \begin{observation}
% Let $\rho$ be the maximum pairwise correlation in $\widetilde{S}$. If $\Delta \sigma_S \geq \delta$, then $\rho \leq \kappa$, where $\kappa = f(\delta)$. 
% \end{observation}
% \begin{observation}\label{Obs1}
% $\Delta \sigma_S \leq \rho$,
% where $ \rho = \frac{\min\limits_{i \in [1,k]}-\sum_{j=1,j\neq i}^{k}\widetilde{A}_{ij}}{(k-1)}$ is the minimum negative mean of pairwise correlations of each member with other members in the set. 
% \end{observation}

%where $ \rho = \frac{\sum_{i=1}^{k}\sum_{j=1,j \neq i}^{k}\widetilde{A}_{ij}}{k(k-1)}$ is the mean of pairwise correlation strengths between the members of $\widetilde{S}$.
%We empirically verified both of the above observations on as many correlation matrices as we could and found out that it always turns out to be true. Specifically, we considered all correlation matrices of $3 x3$ that were generated at a numerical resolution of 0.01. However, as size of the correlation matrix grows bigger, it gets computationally infeasible to cover all correlation matrices at higher numerical resolution. Therefore, we generated a population of around 1,000,000 correlation matrices of size $k \times k$ for $k = 4,5,6$. Each correlation matrix of size $k \times k$ is generated by randomly selecting $k(k-1)/2$ numbers in the range $[s,e]$ under uniform distribution, where $s\in [-1,1]$ and $e\in [s,1]$, and then arbitrary placing them as the off-diagonal entries in the upper triangular part of the matrix. The lower triangular part is then filled to keep the matrix symmetric. The resultant matrix is then checked for positive semi-definiteness before being considered as a valid correlation matrix. 

% \graphicspath{{Methods/Figs/}}



%Both of the above observations could be leveraged to significantly cut down the search space for finding multipoles with stronger linear gain.
 

%Specifically, Observation~\ref{Obs0} implies that the linear gain is smaller for larger multipoles. Hence, if we are only interested in finding multipoles with linear gain at least $\delta$, we can safely ignore all sets beyond of size $\floor*{\frac{1+\delta}{\delta}}$. 

%Further, Observation~\ref{Obs1} implies that for a set $S$ to have stronger linear gain, all the members in its self-canceling version $\widetilde{S}$ must have stronger negative mean of correlations. Intuitively, such a scenario is more likely to be observed in promising candidates where all the pairwise correlations in $\widetilde{S}$ are negative.

%$S$ when all the pairwise correlations in $\widetilde{S}$ are negative. We refer to such sets as \emph{\textbf{promising candidates}} of multipoles.

\subsection{Promising Candidates}\label{Sec:PromCand}
\begin{definition}
A set $S$ is said to be a \textbf{promising candidate} if i) $|S| \leq \floor*{\frac{1+\delta}{\delta}}$, where $\delta$ is the user-specified threshold on linear gain, and ii) maximum pairwise correlation in its self-canceling form $\widetilde{S}$ is negative. %$\widetilde{S} <0$. % $\rho_S < 0$.
\end{definition}

Promising candidates can be classified into two types: i) Negative Cliques, and ii) Negative Equivalent Cliques.


%Recall from section~\ref{sec:EmpObs} that flipping the signs of one or more variables in a set does not alter the eigenvalues of the underlying correlation matrix. All promising candidates belong to a family of sets that are transformable into a set where all pairwise correlations are negative. Such a family of sets can be classified into two types: i) Negative Cliques, and ii) Negative Equivalent Cliques.

%In other words, a promising candidate $S$ is one in which all the pairwise correlations among the members of its self-canceling version $\widetilde{S}$ are below 0, and whose maximum size is governed by $\delta$.

%In other words, a promising candidate $S$ is one for which i) $|S| \leq \floor*{\frac{1+\delta}{\delta}}$, and ii)  can be transformed into a set $\widetilde{S}$ where all pairwise correlations are negative, without changing the eigenvalues of underlying correlation matrix. 


% In this work we propose to keep the search for multipoles limited to
% promising candidates for multiple reasons: 1) Such candidates are statistically rarer (as will be further clear in section~\ref{}), hence computational cost of the search goes down dramatically, thereby allowing one to design a computationally feasible algorithm to find multipoles. 2) Multipoles formed in non-promising candidates tend to have smaller linear gain. This is further evident in Figure~\ref{},\ref{} and \ref{} where the red line indicates the highest linear gain observed for a non-promising candidate among all the tested matrices. Hence, all the multipoles that will be missed are likely to have smaller linear gain. Further notice that the red line shifts towards left with increase in the size of the set, which suggests that maximum limit for linear gain of a non-promising candidate decreases with increase in size, which further implies that multipoles of bigger sizes are less likely to be missed for any given threshold $\delta$ on linear gain.

%Promising candidates can be further classified into two classes: i) Negative Cliques, and ii) Negative-Equivalent Cliques.

%  This is further evident from Figure~\ref{} where all red scatter indicating promising candidates are concentrated in the zone of higher linear gain, compared to the blue scatter that indicate all other remaining sets.

%Leveraging the above observation, in this work we propose a family of computationally efficient approaches to find multipoles with stronger linear gains. Our proposed approaches gain computational efficiency by limiting the search space to promising candidates which are much fewer in number. Promising candidates can be classified into two classes: i) Negative Cliques, and ii) Negative Equivalent Cliques.


\begin{definition}\label{def:negcl}
A \textbf{negative clique} refers to a set where all the pairwise correlations between its members are negative.
\end{definition} 

The terminology is motivated from the appearance of such sets in a correlation graph, where each vertex represents a variable and the weight of an edge $e(X_i,X_j)$ is equal to $corr(X_i,X_j)$. Such sets would appear as a clique of negative edges in the correlation graph. It can be shown that the self-canceling form of any negative clique is itself,i.e. $S = \widetilde{S}$, and by definition satisfies the requirement of all pairwise correlations in $\widetilde{S}$ to be negative. Therefore, a negative clique is a promising candidate.

\graphicspath{{Methods/Figs/}}
\begin{figure}[tb]
\centering
\begin{subfigure}[t]{0.15\textwidth}
\includegraphics[width=2.5cm,height=2.5cm]{Pseudo1}
\centering
\caption{Negative-Equivalent clique}
\label{fig:pseudo1}
\end{subfigure}
\centering
\begin{subfigure}[t]{0.15\textwidth}
\includegraphics[width=2.5cm,height=2.5cm]{Pseudo2}
\centering
\caption{Negative clique }
\label{fig:pseudo2}
\end{subfigure}
\caption{Illustrating equivalence between a negative-equivalent clique and a negative clique.}
\label{fig:pseudo}
\end{figure}

\begin{definition}\label{def:pseudo}
A \textbf{negative-equivalent clique} refers to a set $S$ whose self-canceling form $\widetilde{S}$ is a negative clique. %can be transformed into a negative clique by flipping the signs of one or more variables in $S$.
\end{definition}
%Since every negative-equivalent clique $S$ can be transformed into a negative clique using sign-flipping operations, and negative cliques are promising candidates, hence every negative-equivalent clique is also a promising candidate. 

All negative-equivalent cliques can be identified using the following lemma.
\begin{lemma}\label{lem:pseudo}
A set $S$ is a \textbf{negative-equivalent clique} \textit{iff} it can be partitioned into two negative cliques $S_1$ and $S_2$ such that the all the cross correlations between members of $S_1$ and $S_2$ are non-negative.
\end{lemma}
\begin{proof}
See supplemental material. 
%This lemma is a special case of Lemma~\ref{lem:pseudo2} with $\rho = 0$. We defer readers to the proof of Lemma~\ref{lem: pseudo2}
%The proof is exactly the same as that of Lemma~\ref{lem:pseudo2}, which is the generalized version of this lemma.

% Consider a negative clique $S = \{X_1,X_2,...,X_k\}$, where all the pairwise correlations are negative. Let $S$ be partitioned arbitrarily into non-empty subsets $S_1$ and $S_2$. Hence, $S_1$ and $S_2$ will also be negative cliques. Without loss of generality, let us flip the signs of all variables in $S_1$ to obtain $S_1' = \{-X_1,-X_2,...,-X_j\}$. Due to this transformation, all the cross-correlations between $S_1'$ and $S_2$ will flip the signs and hence will become non-negative. Furthermore, every pairwise correlation within $S_1'$ remains negative, since $corr(X,Y) = corr(-X,-Y)$. Also correlations within $S_2$ remain negative. As a result, the negative equivalent set $S'$ can be partitioned into two negative cliques $S_1'$ and $S_2$ with all non-negative cross-correlations between them. Since $S'$ was generated using an arbitrary partitioning of an arbitrary negative clique $S$, this holds true for all negative equivalent cliques. 

% To prove converse, consider a set $S$ that can be partitioned into two negative cliques $S_1$ and $S_2$ such that all pairwise cross-correlations between $S_1$ and $S_2$ are non-negative. Now, let us flip the signs of all variables in any one of the two partitions say $S_1$ (w.l.o.g) to form $S_1'$. Then by similar arguments as above, all pairwise correlations within $S_1'$ and $S_2$ will remain negative, while the cross correlations between $S_1$ and $S_2$ flip their signs from positive to negative. Hence, all the pairwise correlations in the transformed set $S_1'\cup S_2$ are negative, which implies that it is a negative clique, and hence, $S$ is a negative equivalent clique. 
\end{proof}



==> Methods/FindingMultipolesJan2019.tex <==
\section{Finding Multipoles}\label{Sec:FindMul}
 \makeatletter
\newsavebox\myboxA
\newsavebox\myboxB
\newlength\mylenA

\newcommand*\xoverline[2][0.75]{%
    \sbox{\myboxA}{$\m@th#2$}%
    \setbox\myboxB\null% Phantom box
    \ht\myboxB=\ht\myboxA%
    \dp\myboxB=\dp\myboxA%
    \wd\myboxB=#1\wd\myboxA% Scale phantom
    \sbox\myboxB{$\m@th\overline{\copy\myboxB}$}%  Overlined phantom
    \setlength\mylenA{\the\wd\myboxA}%   calc width diff
    \addtolength\mylenA{-\the\wd\myboxB}%
    \ifdim\wd\myboxB<\wd\myboxA%
       \rlap{\hskip 0.5\mylenA\usebox\myboxB}{\usebox\myboxA}%
    \else
        \hskip -0.5\mylenA\rlap{\usebox\myboxA}{\hskip 0.5\mylenA\usebox\myboxB}%
    \fi}
\makeatother


% The problem of maximal multipole discovery from a time series dataset could be formulated as the following:

% \begin{definition}[\textbf{Problem Formulation:}]\label{Def:Prob}
% Find the set $P$ of all maximal multipoles in a given time series dataset. %that shows linear gain at least $\delta$, where $\delta$ is a user-specified threshold.
% \end{definition}

The combinatorial aspect of the problem makes it extremely challenging to come up with an approach that is both computationally efficient and guarantees completeness of the search. A brute-force approach would examine all subsets of size  $k$, varying $k$ from $3$ to $N$, the total number of time series in the dataset. While such an approach guarantees completeness of the search, it will easily become computationally infeasible even for very small datasets due to its exponential time complexity. To give an estimate, one of our real-world datasets is quite small in size and has only 171 time series. However, performing a brute-force search on a regular desktop over all subsets of i) size 4 takes about 4 hours, ii) size 5 takes more than 5 days, and so on for subsets of size beyond 5. 

In this paper, we propose a correlation graph-based approach to capture most interesting multipoles in a computationally efficient manner. Our approach is primarily motivated by some empirical observations that indicate a direct relationship between the linear gain of a set and the strengths of pairwise correlations between the members of the set. Leveraging these observations, our approach identifies and restricts the search for multipoles to a family of subsets, which we refer to as `promising candidates` that are more likely to exhibit multipole relationships with stronger linear gain between their members. Such a family of subsets are usually much rarer in the data, thereby contributing to the remarkably high computational efficiency of our approach,  although with some loss of completeness in the final output of multipoles, especially at lower thresholds on linear gain. 

In the remainder of this section, we first define a canonical form for a set of variables called \textit{self-canceling} form that has linear dependence and linear gain identical to that of the original set. We then present our empirical observations that indicate an inverse relationship between linear gain of a set and the largest pairwise correlation in its canonical form. Finally, we describe how the empirical observations can be leveraged to identify promising candidates for multipoles and describe our proposed approach in detail.


%In the remainder of this section, we first define a canonical form for a set of variables called \textit{self-canceling} form that has linear dependence and linear gain identical to that of the original set. Based on the defined canonical form, we then present our empirical observations that indicate an inverse relationship between linear gain of a set and the largest pairwise correlation in its self-canceling form. Finally, we describe how the empirical observations can be leveraged to identify promising candidates for multipoles and present a detailed description of our proposed approach.


%Before describing our approach in detail, we first present the empirical observations that we will use to identify promising candidates. 


%Let the correlation matrix of $\textcircumacute{S}$ be denoted by $\textcircumacute{A}$. 


%\input{Methods/TheoreticalBounds}
%\input{Methods/EmpiricalBounds}
\input{Methods/EmpiricalBoundsJan2019}
% \input{Methods/ProposedApproach}
\input{Methods/ProposedApproachMaximal}
\input{Methods/comet_extendedJan2019.tex}

% Move to supplemental material
%\input{Methods/TimeComplexity}

==> Methods/ProposedApproachMaximal.tex <==
\subsection{Proposed Approach: CoMEt}\label{sec:COMET}
Leveraging the above empirical observations and the concept of promising candidates discussed in previous section, we propose our \textbf{C}lique Based \textbf{M}ultipole S\textbf{E}arch (\textbf{CoMEt}) to find multipoles. The central idea of CoMEt is to find all promising candidates for multipoles (negative cliques and negative-equivalent cliques) and then check each of them to obtain true multipoles. To find all promising candidates, we first construct a graph such that every promising candidate forms a clique in it. We then obtain all maximal promising candidates by enumerating all the maximal cliques of the constructed graph. Note that maximal clique-enumeration problem is NP-complete in general. However, the cliques of our interest tend to be rare in the graphs generated from real-world datasets, which allows us to recover most of the promising candidates in much less computing time. For each maximal clique obtained, we examine its subcliques and select all those that form true multipoles. Finally we eliminate all duplicate and non-maximal multipoles to obtain the final set of maximal multipoles.
%Note that maximal clique-enumeration problem is NP-complete in general. However, the cliques of our interest tend to be rare in the graphs generated from real-world datasets, which allows us to recover most of the promising candidates in much less computing time. 

Algorithm~\ref{Algo:Comet} summarizes the CoMEt approach. We begin by finding all maximal promising candidates in line 3, viz. maximal negative cliques and maximal negative-equivalent cliques using Algorithm~\ref{Algo:PromCand}. Among the obtained maximal promising candidates, we then obtain all the multipoles in line 3 using Algorithm~\ref{Algo:BreakCliq}. Finally, in line 5, we eliminate duplicate and non-maximal multipoles using Algorithm~\ref{Algo:RemDupl}. We next describe each of the modules used in the different steps of CoMEt. 

\begin{algorithm}[!h]
\footnotesize
  \caption{CoMEt (\textbf{C}lique Based \textbf{M}ultipole S\textbf{e}arch)}\label{Algo:Comet}
  \begin{algorithmic}[1]
  \Statex{\textbf{Input} Dataset:$\mathcal{D}$, Parameters: $\sigma$,$\delta$}
  \Statex{\textbf{Output} set $U$ of maximal multipoles with linear gain $\geq \delta$.}
  \State{$C \gets $ FIND PROMISING CANDIDATES($D$)}
%   \State{$N \gets $ FIND NEGATIVE CLIQUES($D$)}
%   \State{$P \gets $ FIND PSEUDO-NEGATIVE CLIQUES($D$)}
%   \State{$C = N \cup P$}
  \For{each clique $S$ in $C$}
    \State{$U \gets$ GET MULTIPOLES FROM CANDIDATE($S$)}
    % \State{$U \gets$ EXTRACT MULTIPOLE($c$)}\Comment{CoMEtFast only}
  \EndFor{}
  
%   \Statex{\textbf{Step 3}: Iterative updates on tripoles with weaker jump}
  \State $U \gets $ REMOVE DUPLICATES \& NON-MAXIMALS($U$)
  \State \textbf{return} $U$
    % \EndProcedure
  \end{algorithmic}
\end{algorithm}

\subsubsection{\textbf{FIND MAXIMAL PROMISING CANDIDATES}}
This module is used to find all maximal promising candidates in the data that include all negative and negative-equivalent cliques. Algorithm~\ref{Algo:PromCand} summarizes this module. The key idea is to construct a correlation graph (network) $G$ (lines 1-4) such that a set of nodes of size $\geq 3$ in $G$ would form a clique iff it is a negative clique or negative-equivalent clique. To accomplish that, we first construct two identical graphs $G_1$ and $G_2$, such that for both graphs, a set of nodes will form a clique iff it is a negative clique. To obtain such graphs, we begin by creating a set  $V_1 = \{v_{11},v_{12},...,v_{1n}\}$ of $n$ nodes such that each node $v_{1i}$ corresponds to a time series $X_i$ in the given dataset $D$. For any pair of nodes  $(v_i,v_j)$, an edge is drawn iff $corr(X_i,X_j) \leq 0$. Let $E_1$ denote the set of all such edges. Then $G_1 = (V_1,E_1)$ is the desired correlation graph where a clique will be formed among a set of nodes iff their corresponding variables in $D$ form a negative clique. Similarly, an identical correlation graph $G_2 = (V_2,E_2)$ can be constructed on a set of nodes $V_2 = \{v_{21},v_{22},...,v_{2n}\}$, where each node $v_{2i}$ corresponds to a time series $X_i$ in the given dataset $D$. 

Next, to include edges for non-negative correlations in all negative-equivalent cliques, we construct a set $E$ of cross-edges between nodes of $G_1$ and $G_2$. Specifically, we connect each node $v_{1i} \in V_1$ to all the nodes $v_{2j} \in V_2$ such that $corr(X_{i},X_{j}) \geq 0$. As a result of this operation, for any negative-equivalent clique $S = S_1 \cup S_2$, where $S_1$ and $S_2$ are its two negative subcliques, all the non-negative correlations across $S_1$ and $S_2$ are now included. Hence, in the resultant graph $G = (V_1 \cup V_2,E_1 \cup E_2 \cup E)$, every negative-equivalent clique will also appear as a clique. Also note that every clique $S$ of size $\geq 3$ in $G$ would be a promising candidate; it would either be a negative clique (if $S \subset G_1$ or $S \subset G_2$), or a negative-equivalent clique (if it includes nodes from both $G_1$ or $G_2$).

From the resultant graph $G$, all the maximal promising candidates could be obtained by enumerating all maximal cliques in graph $G$ using any of the standard clique-enumeration algorithms. In this work, we used an efficient algorithm proposed in \cite{eppstein2011listing} (line 11) to enumerate maximal cliques in sparse graphs (implementation provided by authors in \cite{cliquecode}). 

%Hence, we can obtain all promising candidates by applying any of the standard clique-search algorithms on $G$ to obtain all cliques. For this work, we used Bron-Kerbosch algorithm \cite{bron1973algorithm} (line 11), which can be used to find all maximal cliques in an undirected and unweighted graph. 

\begin{algorithm}[!h]
\footnotesize
  \caption{FIND MAXIMAL PROMISING CANDIDATES}\label{Algo:PromCand}
  \begin{algorithmic}[1]
  \Statex{\textbf{Input} Dataset:$\mathcal{D}$,$\rho$} \Comment{$\rho = 0$ for CoMEt}
  \Statex{\textbf{Output} set $C$ of all maximal promising candidates}
  \Statex{\textbf{Correlation Graph Construction:}}
  \State{$V_1 \gets$ set of $n$ vertices $v_{11},v_{12},...,v_{1n}$  corresponding to $n$ variables $X_1,X_2,...,X_n$ in $D$}
  \State{$E_1 \gets$ All pairs $(v_{1i},v_{1j})$ s.t. $corr(X_i,X_j) \leq 0$}  %\Comment{$\rho = 0$ for CoMEt}
  \State{$G_1 = (V_1,E_1)$}
  \State{$G_2 = (V_2,E_2)$ be the exact duplicate of $G_1$}
  \State{$E \gets \phi$} \Comment{An empty set of edges}
  \For{each $v_{1i} \in V_1$}
        \State{$E' \gets$ all pairs $(v_{1i},v_{2j})$ s.t. $corr(X_i,X_j) \geq 0$} %\Comment{$\rho = 0$ for CoMEt}
        \State{$E = E \cup E'$}
  \EndFor
  \State{$G = (V_1 \cup V_2,E_1 \cup E_2 \cup E)$}
  \State{$C \gets$ All maximal cliques of $G$} \Comment{algorithm proposed in \cite{eppstein2011listing}}
  \State{Remove all duplicate maximal cliques from $C$}
%   \State{$C \gets $ All cliques in $C$ with smallest index node in $V_1$} \Comment{Remove duplicate cliques}
  \State \textbf{return} $C$
  \end{algorithmic}
\end{algorithm}



Note that every maximal promising candidate will result in formation of two maximal cliques in $G$. For instance, every negative clique will form two cliques: one in $G_1$ and $G_2$ each. Similarly, a negative-equivalent clique $S = (S_1 = \{X_i,X_j\},S_2 = \{X_k\})$, where $S_1$ and $S_2$ are two negative sub-cliques, will result in formation of two cliques: $(v_{1i},v_{1j},v_{2k})$ and $(v_{2i},v_{2j},v_{1k})$ in $G$. For every maximal promising candidate, exactly one of the maximal cliques is retained (line 12). Finally, the set of retained maximal cliques is returned as the set of all maximal promising candidates.

 

% \subsubsection{\textbf{FIND NEGATIVE CLIQUES:}}
% This module is used to find all negative cliques in the data. The module is summarized in Algorithm~\ref{Algo:NegCliq}. The key idea is to first construct a graph $G$ (lines xx-xx) such that a set of nodes in $G$ would form a clique iff it is a negative clique. To construct $G$, we consider a set $V = \{v_1,v_2,...,v_n\}$ of $n$ vertices such that each vertex corresponds to a time series in the given dataset $D$. For any pair of vertices  $(v_i,v_j)$, an edge is drawn iff $corr(X_i,X_j) \leq 0$.   
% On the resultant graph $G$, one can then apply any of the standard clique finding algorithms to obtain all the negative cliques. For this work, we used Bron Kerbosch algorithm \cite{} (line xx) that can be used to find all maximal cliques in an undirected and unweighted graph.

% \subsubsection{\textbf{FIND negative-equivalent CLIQUES:}}
% This module is used to find all negative-equivalent cliques in the data. Algorithm~\ref{Algo:PseudoNeg} summarizes the entire module. The key idea is same as that of FIND NEGATIVE CLIQUES, except that this time we construct a different graph $G$ that will also include pseudo-negative cliques in the graph as shown in lines xx-xx. We first construct two copies $G_1 = (V_1,E_1)$ and $G_2 = (V_2,E_2)$ of the same graph that was constructed in Algorithm~\ref{Algo:NegCliq} to find negative cliques. As a result, every variable $X_i$ has two representative vertices $v_{1i}$ in $G_1$ and $v_{2i}$ in $G_2$ respectively. 

% On the resultant graph $G$, one can then apply any of the standard clique finding algorithms to obtain all the negative cliques. For this work, we used Bron Kerbosch algorithm \cite{} (line xx) that can be used to find all maximal cliques in an undirected and unweighted graph.

%Although the problem is NP-hard, many efficient algorithms have been proposed to find all cliques in the graph. In this work, we used one of the most popular Bron Kerbosch algorithm \cite{} that finds all the cliques in the graph.

% \begin{algorithm}[!h]
% \footnotesize
%   \caption{FIND NEGATIVE CLIQUES}\label{Algo:NegCliq}
%   \begin{algorithmic}[1]
%   \Statex{\textbf{Input} Dataset:$\mathcal{D}$}
%   \Statex{\textbf{Output} set $N$ of all maximal negative cliques}
%   \Statex{Graph Construction:}
%   \State{$V \gets$ set of $n$ vertices $v_1,v_2,...,v_n$ corresponding to $n$ variables $X_1,X_2,...,X_n$ in $D$}
%   \State{$E \gets$ All pairs $(v_i,v_j)$ such that $corr(X_i,X_j) \leq 0$}
%   \State{$G = (V,E)$}
%   \State{$N \gets$ All maximal cliques of $G$} \Comment{using Bron-Kerbosch Algorithm}
%   \State \textbf{return} $N$
%   \end{algorithmic}
% \end{algorithm}

\subsubsection{\textbf{GET MULTIPOLES}} This procedure is applied to each of the obtained maximal promising candidates to extract all multipole relationships. As summarized in Algorithm~\ref{Algo:BreakCliq}, we begin by checking if the given candidate $S$ forms a multipole by comparing its linear dependence and linear gain with user-specified thresholds $\sigma$ and $\delta$, respectively. If so, then $S$ is added to the set of discovered multipoles and we move on to the next promising candidate. Otherwise, it could be possible that one or more of the subsets of $S$ might form a multipole that satisfies the thresholds. However, if $\sigma_S$ turns out to be lower than the threshold $\sigma$, then by Lemma~\ref{lem:ld}, all the subsets of $S$ would also have weaker linear dependence than $\sigma$ and thus, could be safely ignored. Therefore, only if $\sigma_S \geq \sigma$, do we perform an exhaustive search on all subsets of $S$ of sizes $[3,\floor*{\frac{1+\delta}{\delta}}]$ and select all the ones that satisfy the thresholds. The range of sizes of subsets is derived based on the observation made in section~\ref{sec:EmpObs}, which states that for a given threshold $\delta$ on linear gain, all sets of sizes beyond $\floor*{\frac{1+\delta}{\delta}}$ can be safely discarded. 
%Hence, and select all the ones that show linear gain stronger than $\delta$. 

Applying the above procedure to all maximal promising candidates might result in inclusion of several non-maximal multipoles in the output. Furthermore, a multipole could be generated multiple times from different maximal promising candidates. Hence, in the final step of CoMEt, we eliminate all non-maximal and duplicate multipoles using the module described below.

\begin{algorithm}
\footnotesize
  \caption{GET MULTIPOLES FROM CANDIDATE(S)}\label{Algo:BreakCliq}
  \begin{algorithmic}[1]
  \Statex{\textbf{Input:} set $S$, $\sigma$, $\delta$}
  \Statex{\textbf{Output} All multipoles $S'$ with $\sigma_{S'} \geq \sigma$, and $\Delta \sigma_{S'} \geq \delta$}
  \If{$\Delta\sigma_S \geq \delta$ and $\sigma_{S'} \geq \sigma$}
    \State{ $M \gets$ S}
  \ElsIf{$\sigma_{S'} \geq \sigma$}
    \State{$M \gets$ all subsets $S'$ of $S$ s.t. $|S'| \in [3,\floor*{1+\frac{1}{\delta}}]$, $\sigma_{S'} \geq \sigma$, and $\Delta \sigma_{S'} \geq \delta$}
  \EndIf
  \State{return $M$}
  \end{algorithmic}
\end{algorithm}


\subsubsection{\textbf{REMOVE NON-MAXIMALS \& DUPLICATES}} This module is called in line 5 of Algorithm~\ref{Algo:Comet} to eliminate all non-maximal and duplicate multipoles that are generated in the previous step. As described in Algorithm~\ref{Algo:RemDupl}, we first initialize two empty sets (lines 1-2): i) $U'$ that collects the final set of non-redundant multipoles, and ii) $IsIncluded$, that maintains a collection of all the subsets of multipoles that are included in the final set $U'$ at any point of time. We then scan through all the multipoles in input set $U$. For each multipole $S$ in $U$, we first check if it is  present in the $IsIncluded$ set, and if not, insert it into the final output set $U'$ as well as insert all the subsets of $S$ in $IsIncluded$ that are not previously present in it (lines 5-8). We then remove $S$ from $U$ and repeat the entire procedure in lines (4-9) until $U$ is empty. All the multipoles in the resultant set $U'$ are consequently distinct and maximal.


% OLD
%\subsubsection{\textbf{REMOVE NON-MAXIMALS \& DUPLICATES:}} This module is called in line 5 of Algorithm~\ref{Algo:Comet} to eliminate all non-maximal and duplicate multipoles that are generated in the previous step. As described in Algorithm~\ref{Algo:RemDuplOld}, we begin with selecting the largest multipole $S$ from $U$, and add it to the final output set $U'$ (lines 3-4) that was originally initialized to an empty set (line 1). We then eliminate all multipoles from $U$ that are either duplicates of $S$ (including $S$ itself) or proper subsets of $S$ (lines 5-6). The entire procedure in lines (3-6) is then repeated until $U$ is empty. All the multipoles in the resultant set $U'$ are consequently distinct and maximal.


\begin{algorithm}
\footnotesize
  \caption{REMOVE DUPLICATES \& NON-MAXIMALS}\label{Algo:RemDupl}
  \begin{algorithmic}[1]
  \Statex{\textbf{Input:} a set $U$ of multipoles}
  \Statex{\textbf{Output:} a set $U'$ of non-maximal and distinct multipoles}
  \State{$U' \gets \phi$} 
  \State{$IsIncluded \gets \phi$}
  \While{$U \neq \phi$}
    \State{$S \gets $ A multipole in $U$}
    \If{$S$ not in $IsIncluded$}
        \State{Insert $S'$ to $IsIncluded$ $\forall S' \subseteq S$}
        \State{$U' \gets U' \cup S$}
    \EndIf
    \State{$U \gets U - S$}
  \EndWhile
  \State{return $U'$}
  \end{algorithmic}
\end{algorithm}


% \begin{algorithm}
% \footnotesize
%   \caption{REMOVE DUPLICATES \& NON-MAXIMALS}\label{Algo:RemDuplOld}
%   \begin{algorithmic}[1]
%   \Statex{\textbf{Input:} a set $U$ of multipoles}
%   \Statex{\textbf{Output:} a set $U'$ of non-maximal and distinct multipoles}
%   \State{$U' \gets \phi$}
%   \While{$U \neq \phi$}
%     \State{$S \gets $ Largest multipole in $U$}
%     \State{$U' \gets U' \cup S$}
%     \State{$W \gets$ all multipoles in $U$ that are duplicates or subsets of $S$}
%     \State{$U \gets U - W$}
%   \EndWhile
%   \State{return $U'$}
%   \end{algorithmic}
% \end{algorithm}



==> Methods/TheoreticalBounds.tex <==
\subsection{Theoretical Bounds on Linear Gain}\label{sec:ThBounds}
 In this section, we present a series of theoretical upper bounds on the linear gain of a multipole.
 
%  In this section, we present a series of theoretical upper bounds on the linear gain of a multipole. 

% empirical and theoretical bounds on linear gain. All the observations presented here will be a key to design an efficient approach to mine multipoles from a given time series data. 
%%%%%%
% Consider a set $S$ of $k$ variables and its correlation matrix $A$. Let $\lambda$ be the least eigenvalue of A. Let $A_{j}$ be the correlation matrix of a subset of $k-1$ variables that is formed by eliminating 

% Consider a block matrix $B = 
% \begin{bmatrix}
% \xoverline{A_{jj}} &C_{j}\\
% C_{j}^T &1\\
% \end{bmatrix}$, where $\xoverline{A_{jj}}$ is the $k-1 \times k-1 $ sub-correlation matrix of a subset of $(k-1)$ variables, $C_{j}$ and $C_{j}^T$ denote the $j^{th}$ column and row vector of $A$ respectively.  Let $\lambda$ and 
% $v = \begin{bmatrix} \xoverline{v_{j}} \\ v_{j}\end{bmatrix}$ be the least eigenvalue and corresponding unit eigenvector of A, where $ \xoverline{v_{j}$ is a $(k-1) \times 1$ vector storing the weights of first (k-1) variables in $v$, and $v_{j}$ denote the weight of $k^{th}$ variable in $v$. Let $\mu$ be the eigenvalue of $\xoverline{A_{jj}}$ and $\Delta \lambda_{j} = \mu - \lambda$ be the increase in eigenvalue due to elimination of $j^{th}$ column and row. Then an upper bound on $\Delta \lambda$ can be obtained as per the following theorem:

% %%%%%%
Consider a set $S= \{X_1,X_2,...,X_k\}$ of $k$ variables and its correlation matrix $A$. Let the block matrix representation of $A = 
\begin{bmatrix}
\xoverline{A_{jj}} &C_{j}\\
C_{j}^T &1\\
\end{bmatrix}$, where $\xoverline{A_{jj}}$ is the $k-1 \times k-1 $ sub-correlation matrix of a subset of $(k-1)$ variables that excludes $X_j$, $C_{j}$ is a $(k-1) \times 1$ vector with $C_{j}[i] = A[i][j]$. Let $\lambda$ and $v = \begin{bmatrix} \xoverline{v_{j}} \\ v_{j}\end{bmatrix}$ be the least eigenvalue and corresponding unit eigenvector of A, where $v_{j}$ denote the weight of $j^{th}$ variable in $v$, and $ \xoverline{v_{j}}$ is a $(k-1) \times 1$ vector storing the weights of remaining (k-1) variables in $v$. Let $\mu$ be the eigenvalue of $\xoverline{A_{jj}}$ and $\Delta \lambda_{j} = \mu - \lambda$ be the increase in eigenvalue due to elimination of $j^{th}$ column and row. Then an upper bound on $\Delta \lambda$ can be obtained as per the following theorem:

%and let $\Delta \lambda_j = \mu - \lambda$ denote the increase in eigenvalue due to elimination of $k^{th}$ column and row. Then an upper bound on $\Delta \lambda_j$ can be obtained as per the following theorem:

% %\alpha_j$, where $\alpha_j =  \sqrt{\frac{\sum_{i=1}^{n}A_{ij}^2}{n-1}}$. 

\begin{theorem}\label{theo1}
$\Delta \lambda_j \leq \lVert C_{j} \rVert \leq \lVert C_{j} \rVert_{1}$ 
\end{theorem}
\begin{proof}
 We have,
\begin{align}\label{eigeq1}
\begin{bmatrix} \xoverline{A_{jj}} &C_{j}\\ C_{j}^T &1\\ \end{bmatrix}\begin{bmatrix} \xoverline{v_{j}} \\ v_{j}\end{bmatrix} &= \lambda \begin{bmatrix} \xoverline{v_{j}} \\ v_{j}\end{bmatrix}. 
\end{align}
First considering the upper half of equation~\ref{eigeq1}, we get
\begin{align*}
    \xoverline{A_{jj}}\xoverline{v_{j}} + C_{j}v_{j} = \lambda \xoverline{v_{j}}
\end{align*}
Or,
\begin{align*}
    C_{j}v_{j} = \lambda \xoverline{v_{j}} - \lVert \xoverline{v_{j}}\rVert \xoverline{A_{jj}}e_{1}\rVert
\end{align*}
where, $e_1 = \frac{\xoverline{v_{j}}}{ \lVert \xoverline{v_{j}}\rVert}$ is the unit vector in the direction of $ \xoverline{v_{j}}$. 

Taking $L2$ norm on both sides, we get
\begin{align*}
    \lVert C_{j}v_{j} \rVert = \lVert \lambda \xoverline{v_{j}} - (\lVert \xoverline{v_{j}}\rVert \xoverline{A_{jj}}e_{1}) \rVert
\end{align*}
For any two vectors $\mathbf{a}$ and $\mathbf{b}$, we have  $\lVert \mathbf{a} \rVert \lVert \mathbf{b} \rVert \geq \mathbf{a}.\mathbf{b}$. Hence, 
\begin{align*}
    \lVert C_{j} \rVert \lVert v_{j} \rVert \geq \lVert \lambda \xoverline{v_{j}} - \lVert \xoverline{v_{j}}\rVert (\xoverline{A_{jj}}e_{1}) \rVert
\end{align*}

For any two vectors $\mathbf{a}$ and $\mathbf{b}$, we have  $$\lVert \mathbf{a} - \mathbf{b} \rVert \geq |\lVert \mathbf{a} \rVert - \lVert\mathbf{b}\rVert |$$. Hence, 

\begin{align}\label{eq_upperhalf1}
    \lVert C_{j} \rVert \lVert v_{j} \rVert \geq |\lambda \lVert  \xoverline{v_{j}} \rVert- (\lVert \xoverline{v_{j}}\rVert) (\lVert \xoverline{A_{jj}}e_{1} \rVert) |
\end{align}
Let $u$ be the unit eigenvector corresponding to the least eigenvalue $\mu$ of $\xoverline{A_{jj}}$. Then, 
$$\lVert \xoverline{A_{jj}}u \rVert = \mu \leq \lVert \xoverline{A_{jj}}e_{1} \rVert $$. Also $\lambda \leq \mu$.
Hence, we can write Eq~\ref{eq_upperhalf1} as 

\begin{align*}
    \lVert C_{j} \rVert \lVert v_{j} \rVert \geq (\mu - \lambda) \lVert  \xoverline{v_{j}} \rVert = \Delta \lambda_j \lVert  \xoverline{v_{j}} \rVert
\end{align*}

Since $v$ is a unit eigenvector. Therefore, $\lVert \xoverline{v_{j}}\rVert = \sqrt{1-v_{j}^2}$. Hence, we can also write

\begin{align} \label{eq_upperhalf2}
    \Delta \lambda_j \lVert  \leq \lVert C_{j} \rVert \sqrt{\frac{v_{j}^2}{1-v_{j}^2}}
\end{align}

Now considering the lower half of equation~\ref{eigeq1}, we can write
\begin{align*}
    C_{j}^T\xoverline{v_{j}} + v_{j} &= \lambda v_{j}
\end{align*}
Or, 
\begin{align*}
    C_{j}^T\xoverline{v_{j}} &= (\lambda -1) v_{j}
\end{align*}
Taking absolute values on both sides, we get
\begin{align*}
     |C_{j}^T\xoverline{v_{j}}|  &= |(\lambda -1)|  |v_{j}|
\end{align*}
For any two vectors $\mathbf{a}$ and $\mathbf{b}$, we have  $\lVert \mathbf{a} \rVert \lVert \mathbf{b} \rVert \geq |\mathbf{a}.\mathbf{b}|$. Hence, 
\begin{align}\label{eq_lowhalf1}
    \lVert C_{j}^T\rVert \lVert \xoverline{v_{j}} \rVert  &\geq |(\lambda -1)||v_{j}|
\end{align}

Note that $\lambda \in [0,1]$. Therefore, we can write 
\begin{align*}
   \lVert C_{j}^T\rVert \lVert \xoverline{v_{j}} \rVert   &\geq (1-\lambda) |v_{j}|
\end{align*}


Let $\Delta \lambda_j = \mu - \lambda$, where $\mu$ is the least eigenvalue of $\xoverline{A_{jj}}$. Hence $\Delta \lambda_j \leq (1-\lambda)$. Using this result in Eq~\ref{eq_lowhalf1}, we get

\begin{align}\label{eq_lowhalf2}
   \lVert C_{j}^T\rVert \frac{\lVert \xoverline{v_{j}} \rVert}{|v_{j}|} = \lVert C_{j}^T\rVert \sqrt{\frac{1-v_{j}^2}{v_{j}^2}}  &\geq \Delta \lambda_j
\end{align}


From Eqs~\ref{eq_upperhalf2} and \ref{eq_lowhalf2} and the fact that $\lVert x \rVert \leq \lVert x \rVert_1$ for any vector $x$, we get
\begin{align*}
    \Delta \lambda_j \leq \lVert C_{j} \rVert \leq \lVert C_{j} \rVert_1
\end{align*}
\end{proof}

Using Theorem~\ref{theo1}, we next present two bounds on the linear gain $\Delta \lambda_S$ of the multipole. 

\begin{corollary}
 $\Delta \lambda_S \leq \sqrt{\frac{\sum_{i=1}^{n}\sum_{j=1,j \neq i}^{n}A_{ij}^2}{k}}$.
\end{corollary}
\begin{proof}
From Theorem~\ref{theo1}, we get
$$\Delta \lambda_j \leq \lVert C_{j} \rVert = \sqrt{\sum_{i=1,i \neq j}^{k}A_{ij}^2} \forall j \in [1,k]$$.

Or,
$$\Delta \lambda_{j}^2 \leq \sum_{i=1,i \neq j}^{k}A_{ij}^2 \forall j \in [1,k]$$.

Hence, writing the above result for all columns and adding them together, we get
$$\sum_{j=1}^{k}\Delta \lambda_{j}^2 \leq \sum_{j=1}^{k}\sum_{i=1,i\neq j}^{k}A_{ij}^2$$
Since $\Delta \lambda_S = min_{j \in [1,k]\Delta \lambda_j}$. Hence,

$$k\Delta \lambda_S^2 \leq \sum_{j=1}^{k}\Delta \lambda_{j}^2 \leq  \sum_{j=1}^{k}\sum_{i=1,i\neq j}^{k}A_{ij}^2$$
Or,
$$\Delta \lambda_S^2 \leq \frac{\sum_{j=1}^{k}\sum_{i=1,i\neq j}^{k}A_{ij}^2}{k}$$
Or,
$$\Delta \lambda_S \leq \sqrt{\frac{\sum_{j=1}^{k}\sum_{i=1,i\neq j}^{k}A_{ij}^2}{k}}$$

\end{proof}

We next present a further tighter bound on $\Delta \lambda_S$  which bounds $\Delta \lambda_S$ by root mean square of off-diagonal entries of at least one of the columns.  

\begin{corollary}
$\exists j \in [1,n]$ such that  $\Delta \lambda_S \leq \sqrt{ \frac{\sum_{i=1}^{k}A_{ij}^2-1}{k-1}}$. 
\end{corollary}
\begin{proof}

From Eq~\ref{eq_upperhalf2}, we get 

\begin{align*}
\Delta \lambda_j \leq \lVert C_{j} \rVert \sqrt{\frac{v_{j}^2}{1-v_{j}^2}} \forall j \in [1,k] 
\end{align*}
%The term $ \sqrt{\frac{v_{j}^2}{1-v_{j}^2}}$ is a monotonically increasing function of $v_j$ for $v_j \in [0,1]$. 
Since $v$ is a unit eigenvector. Hence $\sum_{i=1}^{k}v_{i}^2 = 1$. By Pigeon Hole Principle, $\exists j \in [1,k]$ such that $|v_j| \leq \frac{1}{\sqrt{k}}$. Also note that the term $ \sqrt{\frac{v_{j}^2}{1-v_{j}^2}}$ in RHS of Eq~\ref{eq_upperhalf2} is a monotonically increasing function of $v_j$ for $v_j \in [0,1]$. Hence, $\exists j \in [1,k]$ such that 
\begin{align*}
   \sqrt{\frac{v_{j}^2}{1-v_{j}^2}} \leq \sqrt{\frac{1/k}{1-1/k}} = \frac{1}{\sqrt{k-1}}
\end{align*}
Using this result in Eq~\ref{eq_upperhalf2}, we get that $\exists j \in [1,k]$ such that
\begin{align*}
   \Delta \lambda_j \leq  \sqrt{\frac{\lVert C_{j} \rVert}{k-1}} 
\end{align*}
Since $\Delta \lambda_S = min_{j \in [1,k]}\Delta \lambda_k$. Hence,  $\exists j \in [1,k]$ such that
\begin{align*}
    \Delta \lambda_S \leq \sqrt{\frac{\lVert C_{j} \rVert}{k-1}} = \sqrt{ \frac{\sum_{i=1}^{k}A_{ij}^2-1}{k-1}}
\end{align*}


\end{proof}

% Note that permuting the rows and columns in any matrix $A$, does not affect the eigenvalue and eigenvectors as far as the ordering is consistent across rows and columns. Therefore, if we exchange $k^{th}$ row and column with $i^{th}$ row and column to generalize theorem~\ref{theo1} and all the intermediate results (Eqs~\ref{eq_upperhalf1}-\ref{eq_lowhalf2}) to all the columns of $A$. In particular, we can generalize Theorem~\ref{theo1} to 

% \begin{align}\label{theo1_gen}
%     \Delta \lambda_j \leq \lVert C_{j} \rVert \leq \lVert C_{j} \rVert_1
% \end{align}
% where, $C_j$ is a $(k-1) \times 1$ vector with all the off-diagonal entries of $j^{th}$ column of $A$. Similarly, Eq~\ref{eq_upperhalf2} can be generalized to 

==> Methods/comet_extendedJan2019.tex <==
\subsection{CoMEtExtended}\label{Sec:COMETEXT}
In certain cases, the completeness and computational efficiency of CoMEt might be unsatisfactory. For instance, at lower thresholds of linear gain, the obtained set of promising candidates by CoMEt approach could potentially miss some of the interesting multipoles (see Figure~\ref{fig:Comet}). On the other hand, at high thresholds of linear gain, there could potentially be many false positives among promising candidates, which would compromise the computational efficiency. Hence, to overcome these limitations of CoMEt, we further propose \textit{CoMEtExtended}, a generalized version of CoMEt, where we redefine what constitutes a promising candidate and allow user to expand or prune the scope of promising candidates in different scenarios. The ability to adjust the search space helps CoMEtExtended in achieving a better trade-off between computational efficiency and completeness at different thresholds of linear gain (demonstrated further in Section~\ref{Sec:CompEval}) . 

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.20\textwidth}
    % \includegraphics[width=\textwidth]{Results/FigsEvalResultsSLP/ReprodSLP}
    \includegraphics[width = 4.5cm,height = 3cm]{Methods/Figs/CometLimitations}

    \centering
    \caption{}
    \label{fig:Comet}
    \end{subfigure}
    \centering
    \begin{subfigure}[t]{0.20\textwidth}
    % \includegraphics[width=\textwidth]{Results/FigsEvalResultsfMRI/ReprodfMRI}
    \includegraphics[width = 4.5cm,height = 3cm]{Methods/Figs/CometExtendedMotivation}
    \centering
    \caption{}
    \label{fig:CometExt}
    \end{subfigure}
\caption{\textbf{Motivation of CoMEtExtended:} (a) shows the multipoles missed by CoMEt for a given threshold $\delta$ on linear gain, which could be recovered by CoMEtExtended by setting parameter $\rho$ to a higher value as shown in (b).}
\label{fig:CometVsCometExt}
\end{figure}

We first begin with redefining the notion of a promising candidate. Specifically, instead of enforcing that all the pairwise correlations in $\widetilde{S}$ be negative, we require all of them to be below a threshold $\rho$, where $\rho \in [-1,1]$. Likewise, we redefine the notion of negative and negative equivalent cliques as \emph{pseudo-negative} and \emph{pseudo negative equivalent} cliques respectively as the following:

\begin{definition}\label{def:pseudonegcl}
For a given $\rho \in [-1,1]$, a \textbf{pseudo negative clique} refers to a set where all the pairwise correlations between its members are less than or equal to $\rho$.
\end{definition} 

\begin{definition}\label{def:pseudonegeq}
A \textbf{ pseudo negative-equivalent clique} refers to a set $S$ whose self-canceling form $\widetilde{S}$ is a pseudo-negative clique.
\end{definition}

A pseudo negative-equivalent clique can be identified using the following lemma which is a general version of Lemma~\ref{lem:pseudo}. 
\begin{lemma}\label{lem:pseudo2}
A set $S$ is a \textbf{pseudo negative-equivalent clique} \textit{iff} it can be partitioned into two pseudo negative cliques $S_1$ and $S_2$ such that the all the cross correlations between members of $S_1$ and $S_2$ are pseudo non-negative.
\end{lemma}
\begin{proof}
See the Supplemental material.

% The definitions of negative cliques and negative-equivalent cliques need to be modified accordingly so that they can include all the promising candidates.

% Consider a pseudo negative clique $S = \{X_1,X_2,...,X_k\}$, where all the pairwise correlations are $\leq\rho$. Let $S$ be partitioned arbitrarily into non-empty subsets $S_1$ and $S_2$. Hence, $S_1$ and $S_2$ will also be pseudo negative cliques. Without loss of generality, let us flip the signs of all variables in $S_1$ to obtain $S_1' = \{-X_1,-X_2,...,-X_j\}$. Due to this transformation, all the cross-correlations between $S_1'$ and $S_2$ will flip the signs and hence will become $\geq-\rho$.  Furthermore, every pairwise correlation within $S_1'$ remain pseudo negative, since $corr(X,Y) = corr(-X,-Y)$. Similarly, correlations within $S_2$ remain pseudo negative. As a result, the pseudo negative equivalent set $S'$ can be partitioned into two pseudo negative cliques $S_1'$ and $S_2$ with all non-negative cross-correlations between them. Since $S'$ was generated using an arbitrary partitioning of an arbitrary pseudo negative clique $S$, this holds true for all pseudo negative-equivalent cliques. 

% To prove converse, consider a set $S$ that can be partitioned into two pseudo negative cliques $S_1$ and $S_2$ such that all pairwise cross-correlations between $S_1$ and $S_2$ are pseudo non-negative, i.e. $\geq -\rho$. Now, let us flip the signs of all variables in any one of the two partitions say $S_1$ (w.l.o.g) to form $S_1'$. Then by similar arguments as above, all pairwise correlations within $S_1'$ and $S_2$ will remain $\leq \rho$, while the cross correlations between $S_1$ and $S_2$ flip their signs and will now $\leq \rho$. Hence, all the pairwise correlations in the transformed set $S_1'\cup S_2$ are pseudo negative, which implies that it is a pseudo negative clique, and hence, $S$ is a pseudo negative-equivalent clique. 
\end{proof}

% Our proposed approach, CoMEt, limits the search for multipoles to negative cliques and negative-equivalent cliques. As a result, all the multipoles that were formed in non-promising candidates would be missed by CoMEt. To recover such multipoles, we propose CoMEtExtended, which is an extended version of CoMEt where we relax the concept of '`negative clique'' and redefine what constitutes a promising candidate. Specifically, in the current definition of a promising candidate $S$, instead of enforcing that all the pairwise correlations in $\widetilde{S}$ be negative, we require all of them to be below a threshold $\rho$, where $\rho \in [-1,1]$. The definitions of negative cliques and negative-equivalent cliques also need to be modified accordingly so that they can include all the promising candidates. To accomplish that, we first relax the notion of a 'negative' and 'non-negative' edge to '\textbf{pseudo negative}' and '\textbf{pseudo non-negative}' edge respectively and define them as the following:  

%The loss in completeness could be further higher at lower thresholds of linear gain, since many multipoles with weaker linear gain  do not necessarily appear as negative cliques or negative equivalent cliques and consequently get missed. Therefore, to improve completeness at lower thresholds of linear gain, we propose CoMEtExtended, an extended version of our approach, where we generalize the scope of promising candidates to include pseudo-negative cliques, where all the pairwise correlations are allowed to below a threshold instead of being necessarily negative. 

%\textbf{Limitations:} In certain cases, the completeness and computational efficiency of CoMEt might be unsatisfactory. For instance, at lower thresholds of linear gain, the obtained set of promising candidates in CoMEt could potentially miss some of the interesting multipoles. On the other hand, at high thresholds of linear gain, there could potentially be many false positives among promising candidates, which would compromise the computational efficiency. Hence, to overcome these limitations of CoMEt,  we further propose \textit{CoMEtExtended}, a generalized version of CoMEt, which involves an additional parameter that can be tuned to expand or prune the scope of promising candidates beyond negative cliques and negative-equivalent cliques, in order to achieve a better trade-off between computational efficiency and completeness at different thresholds of linear gain.  

%space  we parametrize the notion of \emph{negative clique} to \emph{pseudo negative clique}, which requires all of the pairwise correlations in a set below a threshold $\rho$, where $\rho \in [-1,1]$. The concept of negative equivalent cliques is also modified accordingly (see Definitions~\ref{def:pseudonegcl} and \ref{def:pseudonegeq}). The advantage of CoMEtExtended over CoMEt is that the search space of interesting multipoles can be expanded or pruned by tuning the parameter $\rho$ which allows one to achieve a better trade-off between computational efficiency and completeness.

%A 'pseudo negative' edge is formed between a pair of nodes only if their pairwise correlation is $\leq\rho$. Similarly, a 'pseudo non-negative' edge is formed between a pair of nodes only if their pairwise correlation $\geq -\rho$.
% \begin{definition}\label{def:pseudonegedg}
% For a given $\rho \in [-1,1]$, a \textbf{pseudo negative edge} refers to the edge formed between a pair of nodes only if the correlation between the variables represented by the two nodes is less than or equal to $\rho$.
% \end{definition}

% \begin{definition}\label{def:pseudononnegedg}
% For a given $\rho \in [-1,1]$, a \textbf{pseudo non-negative edge} refer to the edge formed between a pair of nodes only if the correlation between the variables represented by the two nodes is greater than or equal to $-\rho$.
% \end{definition}

% Using the above defined notions of pseudo-negative and pseudo non-negative edges\footnote{Note that for $\rho > 0$, all the edges with correlation strengths $\in [-\rho,\rho]$ will be treated as both pseudo negative and pseudo non-negative edges. The overlap between the two classes of edges is essential for Lemma~\ref{lem:pseudo2} to hold which we will discuss shortly.}, 

Using the above definitions and results, we now propose CoMEtExtended which is the more general version of CoMEt. The steps of CoMEtExtended are exactly the same as that of CoMEt, the only difference being in the lines 2 and 7 of  Algorithm~\ref{Algo:PromCand} where the threshold of 0 on pairwise correlations is replaced by $\rho$ and $-\rho$,  respectively. By incorporating $\rho$ in thresholds, we ensure that every clique in the resultant graph is either a pseudo negative clique or a pseudo negative-equivalent clique. Note that setting $\rho$ to zero  gives us the original definition of promising candidates, whereas setting $\rho$ to a higher positive value would include more sets as promising candidates and hence lead to recovery of more of the missed multipoles (see Figure~\ref{fig:CometExt}). However, it should be noted that setting $\rho$ to positive values would increase the number of candidate cliques and thus increase the computational cost. In fact, setting $\rho$ to 1 would turn CoMEtExtended into an exhaustive brute-force search, which guarantees completeness, but would be computationally infeasible. On the other hand, setting $\rho$ to a high negative value would reduce the search space and hence leads to much faster recovery of the multipoles with a very high linear gain in larger datasets. %In the remainder of this paper, we will refer to CoMETExtended version of our approach by the generic name CoMEt.

% Also note that for any given user-specified threshold $\delta$ on linear gain, there exists a range of values of parameter $\rho$ for which CoMEtExtended is guaranteed to perform a complete search of multipoles. Such a range of values could be obtained with the help of a curve that marks the upper boundary of the distribution of correlation matrices of all sizes, e.g. the black dash line shown in Figure~\ref{fig:CometExt}. 

% For any given user-specified threshold on linear gain, there exists a range of values of parameter $\rho$ for which CoMEtExtended is guaranteed to perform a complete search of multipoles. 

% In particular, a pseudo-negative clique would have all pairwise correlations below $\rho$, whereas the non-negative edges in pseudo negative-equivalent cliques should be $\geq -\rho$.

% In fact, setting $\rho$ to 1, would result in the entire set of variables to be the promising candidate. As a result, the CoMEt would turn into a brute-force search operation albeit with an increment in computational cost. 
